Astropulse: A Search for Microsecond Transient Radio Signals Using Distributed Computing. I. Methodology

We are performing a transient, microsecond timescale radio sky survey, called "Astropulse," using the Arecibo telescope. Astropulse searches for brief (0.4 {\mu}s to 204.8 {\mu}s), wideband (relative to its 2.5 MHz bandwidth) radio pulses centered at 1,420 MHz. Astropulse is a commensal (piggyback) survey, and scans the sky between declinations of -1.33 and 38.03 degrees. We obtained 1,540 hours of data in each of 7 beams of the ALFA receiver, with 2 polarizations per beam. Examination of timescales on the order of a few microseconds is possible because we used coherent dedispersion. The more usual technique, incoherent dedispersion, cannot resolve signals below a minimum timescale. However, coherent dedispersion requires more intensive computation than incoherent dedispersion. The required processing power was provided by BOINC, the Berkeley Open Infrastructure for Network Computing.

==> sens_add.tex <==
Some groups have searched for these primordial black holes (PBHs) in the radio, but many researchers have looked for gamma-ray emission instead \citep{ukw10}.  Radio and gamma-ray surveys make very different assumptions about the PBHs' evaporation time, so that their results are difficult or impossible to compare in a meaningful way.  Ukwatta talks about PBH explosions having timescales of seconds or minutes, whereas Astropulse is looking for microsecond pulses.  This means that Ukwatta's black hole explosions are undetectable by Astropulse, since their flux density is comparatively very low.  On the other hand, Ukwatta's rate limit (the minimum detectable number of events per volume per time) is $10^{-1}$ \pcyr, which is many orders of magnitude worse than Astropulse's rate limit of $1.6 \cdot 10^{-12}$ \pcyr.

